Pirouette: Higher-Order Typed Functional Choreographies

We present Pirouette, a language for typed higher-order functional choreographic programming. Pirouette offers programmers the ability to write a centralized functional program and compile it via endpoint projection into programs for each node in a distributed system. Moreover, Pirouette is defined generically over a (local) language of messages, and lifts guarantees about the message type system to its own. Message type soundness also guarantees deadlock freedom. All of our results are verified in Coq.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "PACMAnon"
%%% End:


==> types.tex <==
\section{Modal Types for Choreographies}
\label{sec:modal-types-chor}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "PACMAnon"
%%% End:

